Tensor Decompositions and Adiabatic Quantum Computing for Discovering Practical Matrix Multiplication Algorithms

Quantum computing and modern tensor-based computing have a strong connection, which is especially demonstrated by simulating quantum computations with tensor networks. The other direction is less studied: quantum computing is not often applied to tensor-based problems. Considering tensor decompositions, we focus on discovering practical matrix multiplication algorithms and develop two algorithms to compute decompositions on quantum computers. The algorithms are expressed as higher-order unconstrained binary optimization (HUBO) problems, which are translated into quadratic unconstrained binary optimization (QUBO) problems. Our first algorithm is decompositional to keep the optimization problem feasible for the current quantum devices. Starting from a suitable initial point, the algorithm discovers tensor decomposition corresponding to the famous Strassen matrix multiplication algorithm, utilizing the current quantum annealers. Since the decompositional algorithm does not guarantee minimal length for found tensor decompositions, we develop a holistic algorithm that can find fixed-length decompositions. Theoretically, by fixing a shorter length than the length for the best-known decomposition, we can ensure that the solution to the holistic optimization problem would yield faster matrix multiplication algorithms.

==> draft_paragraphs.tex <==
AlphaTensor \cite{Fawzi_Balog_Huang_Hubert_Romera_Paredes_Barekatain_Novikov_RRuiz_Schrittwieser_Swirszcz_et_2022} has been an inspiration behind this work. Their idea of using reinforcement learning to solve the problem tackles the crucial problem that persists in the decompositional algorithm in this work. The decompositional approach aims to minimize the main objective presented in Section \ref{prob:main_objective}. Although we are able to minimize this even for relatively large matrices, it is not a sufficient objective in order to produce tensor decompositions with minimal rank. In the reinforcement learning algorithm, our main objective necessarily encodes the short-term reward in AlphaTensor. As we know, minimizing/maximizing short-term reward does not necessarily minimize/maximize long-term reward in reinforcement algorithms. Using the reinforcement learning terminology, we should find a method to encode the long-term reward in the decompositional algorithm. In the decompositional algorithm, we do not have a method to minimize rank in the long-term sense, which is one of the objectives of AlphaTensor. On the other hand, in the holistic algorithm, we aim to solve this problem with the cost that the computational complexity grows too large for the current quantum computers.

The meta-algorithmic nature makes the problem to be more ''static''. Comparing the algorithms in this study to those aimed at finding a marked element from an unsorted list highlights the distinction between static and dynamic problems. In search algorithms, the outcome depends on both the marked element and the input list, constituting dynamic elements. Conversely, in our scenario, the algorithm remains independent of the elements within the matrices (except for the field).

\textbf{Advantageous Quantum Algorithm Design Characteristics.} 
Discovering tensor decompositions and especially matrix multiplication algorithms with quantum computers admits favorable properties from a quantum algorithm design perspective. First, the role of quantum computing in this solution is to work as a meta-algorithm for finding classical algorithms. The input to the algorithms is a simple triple $(n, m, p)$ describing the dimensions of the multiplied matrices, the scalar field ($\mathds{R}$ or $\mathds{Z}_2$), and possibly the length of the decomposition or an initial starting point for discovery. The meta-algorithmic nature makes the problem to be more ''static''. If we compare the algorithms in this work to algorithms for finding a marked element from an unsorted list, we see the difference between static and dynamic problems. In search algorithms, the result depends on the marked element as well as the input list, which are both dynamic elements. In our case, the algorithm does not depend on the elements that the matrices contain (except the field).

Comparison of quantum algorithms to classical algorithms has proved to be hard. In our work, the meta-algorithmic perspective adds a different angle to the comparison. The comparison between quantum and classical versions of this type of algorithm is relatively simple: the quantum algorithm works better if it is able to find a faster matrix multiplication algorithm than any known classical algorithm. Time is not an important measure because of the static and extremely hard nature of the problem. In other words, do we need faster algorithms for rediscovering the current matrix multiplication algorithms? The answer is probably no since this would not immediately advance matrix multiplication algorithms themselves

The second favorable quantum computational feature of the problem is related to its complexity. In our formulation, the algorithms for discovering tensor decompositions and matrix multiplication algorithms are expressed as higher-order unconstrained binary optimization (HUBO) problems. These HUBOs have just hundreds of variables and the number of variables scales linearly with respect to the dimensions of the tensors. Having hundreds or even thousands of variables is not a lot compared to the capabilities of the current classical solvers. For example, CPLEX and Gurobi are able to solve problems consisting of millions of variables and also D-wave claims to support hundreds of thousands of variables (i.e., higher order terms in the binary polynomial). The challenge why classical solvers are not able to solve these problems is because of the high number of interactions.

In the case of quantum optimization frameworks like quantum annealing and QAOA, the number of variables is theoretically equal to the number of qubits. For finding practical quantum advantage in the near term, we want to identify problems that have a low number of variables (qubits) but which are still too hard for classical computers. Thus, practical quantum advantage could be found in problems of having a small number of variables but a high number of complicated interactions between them. This work shows that computing tensor decompositions and matrix multiplication algorithms has those characteristics, which makes it an interesting candidate to study. As \cite{kim_2023} points out, demonstrating the near-term utility of quantum systems over classical counterparts connects to achieving significant entanglement growth. This growth should be of a scale where classical approximations struggle. Essentially, to showcase the utility and advantage of quantum systems, it is crucial to identify suitable problems that rapidly grow in entanglement, outpacing the capabilities of classical computational methods.

The results show that no quantum computer nor classical computer to which we have had access could solve the proposed minimization problems, which is an expected outcome considering the problem's complexity. On the other hand, due to the previous work \cite{Fawzi_Balog_Huang_Hubert_Romera_Paredes_Barekatain_Novikov_RRuiz_Schrittwieser_Swirszcz_et_2022}, we are able to demonstrate that the previously found tensors minimize the objectives correctly. We are also able to rediscover the Strassen algorithm in the case that we have a good initial starting point. In any case, the algorithms produce tensor decompositions, and they could also be utilized in other problems involving tensor decompositions, or they could be part of a quantum-classical algorithm to solve the problem.

There are many interesting directions to develop this work further. We might want to assume that the solutions generally admit certain symmetries as in \eqref{eq:symmetries}. These symmetries reduce the number of variables in the formulations; for example, in the case \eqref{eq:symmetries}, we obtain only half of the number of variables. We are also interested in trying other classical methods to solve the problem. For example, tensor networks and classical non-linear solvers could be useful. In this work, we utilized the Hamming distance, but a natural question would be: Are there other distance metrics that would work better? Another related question is that what happens if we expand the integer set? For example, AlphaTensor \cite{Fawzi_Balog_Huang_Hubert_Romera_Paredes_Barekatain_Novikov_RRuiz_Schrittwieser_Swirszcz_et_2022} assumes that the terms for the tensors are picked between integers -2 to 2. Our model enables easy encoding of larger integer sets. We are also interested in developing quantum-classical systems, for example, a system that would integrate classical machine learning and quantum optimization, as suggested earlier.

==> figures/energy_landscape_example.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{axis}[
    no markers,
    domain=1:9,
    samples=100,
    ymin=0,
    ymax=0.3,
    axis lines*=left,
    xlabel=tensors,
    ylabel=HUBO/QUBO energy,
    height=5cm,
    width=10cm,
    xtick=\empty,
    ytick=\empty,
    enlargelimits=false,
    clip=false,
]

\addplot [smooth, thick] {
    (x < 4) * exp(-((x-5)^2)/(2*1^2))/(1*sqrt(2*pi)) +
    (x >= 4 && x <= 6) * (0.2 + 0.01*x) +
    (x > 6) * exp(-((x-5)^2)/(2*1^2))/(1*sqrt(2*pi))
};

\addplot [only marks, mark=*, mark options={fill=red}] coordinates {(5.98, 0.26)};
\node [pin={[pin distance=0.2cm]45:{$T_{i_0}$}}] at (axis cs:5.98, 0.26) {};

\addplot [only marks, mark=*, mark options={fill=red}] coordinates {(3.98, 0.24)};
\node [pin={[pin distance=0.2cm]45:{$T_{i_1}$}}] at (axis cs:3.98, 0.24) {};

\addplot [only marks, mark=*, mark options={fill=red}] coordinates {(8.9, 0.000198655)};
\node [pin={[pin distance=0.2cm]135:{$T_{S}$}}] at (axis cs:8.9, 0.000198655) {};
v
\addplot [only marks, mark=*, mark options={fill=red}] coordinates {(0.001, 0.001)};
\node [pin={[pin distance=0.2cm]45:{$\mathcal{O}$}}] at (axis cs:0.001, 0.001) {};

\end{axis}
\end{tikzpicture}
    \caption{Example of energy landscape in non-trivial tensor decompositions}
    \label{fig:energy_landscape}
\end{figure}

